Deep Forward and Inverse Perceptual Models for Tracking and Prediction

We consider the problems of learning forward models that map state to high-dimensional images and inverse models that map high-dimensional images to state in robotics. Specifically, we present a perceptual model for generating video frames from state with deep networks, and provide a framework for its use in tracking and prediction tasks. We show that our proposed model greatly outperforms standard deconvolutional methods and GANs for image generation, producing clear, photo-realistic images. We also develop a convolutional neural network model for state estimation and compare the result to an Extended Kalman Filter to estimate robot trajectories. We validate all models on a real robotic system.

==> abstract.tex <==
We consider the problems of learning forward models that map state to high-dimensional images and inverse models that map high-dimensional images to state in robotics tracking and prediction tasks. Specifically, we present a non-parametric perceptual model for generating video frames from state with deep networks, and provide a framework for its use in tracking and prediction tasks. We show that our proposed model greatly outperforms standard deconvolutional methods for image generation, producing clear, photo-realistic images. We also  develop a convolutional neural network model for state estimation and compare the result to an Extended Kalman Filter to estimate robot trajectories.  We validate all model on a real robotic system. %As a comparison, we introduce a secondary framework consisting of a discriminative, inverse model for state estimation, and compare this approach to that using a generative model. 

%\fixed{Possibly too focused on learning the inverse model. I would set up in relation to forward and inverse kinematics.}

% Generative model can be seen as forward kinematics + 2D-3D image projection



==> ekf_description.tex <==
\section{Extended Kalman Filter}

An Extended Kalman Filter \cite{julier1997} can be used to infer the underlying state distributions for nonlinear discrete time systems exhibiting latent Markovian dynamics, assuming Gaussian likelihoods and conjugate priors. In this section, we review the basic EKF formulation for explanatory support. \\
We can describe the equations governing the distributions of state and observation as follows:

\begin{equation}
    x_{t+1} = f\left(x_t\right) + \epsilon_t 
    \qquad 
    \epsilon_t \sim \mathcal{N}(0,Q)
\end{equation}

\begin{equation}
    y_{t+1} = g\left(x_{t+1}\right) + \delta_{t+1} 
    \qquad 
    \delta_{t+1} \sim \mathcal{N}(0,R)
\end{equation} 

with $x \in \mathbb{R}^{n}$ representing the state, $y \in \mathbb{R}^{m}$ the measurement, $f:\mathbb{R}^{n} \mapsto \mathbb{R}^{n}$ the transition function, $g:\mathbb{R}^{n} \mapsto \mathbb{R}^{m}$ the observation function, and respective covariance matrices denoted by $Q\in \mathbb{R}^{n \times n}$ and $R \in \mathbb{R}^{m \times m}$. Note that this formulation assumes the state is governed by drift dynamics alone, without the presence of control input. First-order approximations of the transition function $f$ and observation function $g$ can be made through linearization:

\begin{equation} \label{lin_f}
    x_{t+1} \approx  f(\mu_t) +J_f (x_t - \mu_t) + \epsilon_t
\end{equation}
\begin{equation} \label{lin_g}
    y_{t+1} \approx  g(\mu_{t+1}) +J_g (x_{t+1} - \mu_{t+1}) + \delta_{t+1} 
\end{equation}

where

\begin{equation}
    J_f = \left. \frac{\partial f(x_t)}{\partial x} \right\rvert_{x_t=\mu_t}
    \qquad \in \mathbb{R}^{n \times n}
\end{equation}
\begin{equation}
    J_g = \left. \frac{\partial g(x_t)}{\partial x} \right\rvert_{x_t=\mu_t}
    \qquad \in \mathbb{R}^{m \times n}
\end{equation}

The latent state distribution is propagated forward in time, producing a prediction at time $t+1$, which is successively conditioned on a new measurement. The computations are performed in two distinct steps:

% With the local approximations in Eq.\ref{lin_f} and Eq.\ref{lin_g}, the Gaussian assumption is maintained, and the posterior distribution is estimated by the expectation and covariance. 

% With the first local approximation, the latent state distribution can be propagated forward in time using its canonical parameters. The expectation and covariance predictions can then be made for time $t+1$. The second linearization provides a way to conditions the distribution given a new measurement. This comprises the 

\\
Prediction:
\begin{equation}
    \mu^-_{t+1} = f\left(x_t\right)
\end{equation}
\begin{equation}
    \Sigma^-_{t+1} = J_f\Sigma_tJ^T_f + Q
\end{equation}

Correction:
\begin{equation}
    \mu_{t+1} = \mu^-_{t+1} + \Sigma^-_{t+1}J_g^T(J_g\Sigma^-_{t+1} J_g^T + R)^{-1}\left(y-g\left(\mu^-_{t+1}\right)\right)
\end{equation}
\begin{equation}
    \Sigma_{t+1} = \Sigma^-_{t+1} - \Sigma^-_{t+1}J_g^T(J_g\Sigma^-_{t+1} J_g^T + R)^{-1}J_g\Sigma^-_{t+1}
\end{equation}


The above formulation assumes a continuously-differentiable, generative (as opposed to a discriminative) observation model $g:\mathbb{R}^{n} \mapsto \mathbb{R}^{m} $. Neural network models are particularly amenable to linearization, and an analytical expression for the Jacobian $J_g$ can be readily obtained in an efficient manner (see Section \ref{Jg_comp}).

The dimensionality of the observations makes it impractical to compute $(J_g^T\Sigma^-_{t+1} J_g + R)^{-1}$ directly. Instead, we use a low-rank approximation of $R$, and perform the inversion in projected space:

\begin{equation}
    (J_g^T\Sigma^-_{t+1} J_g + R)^{-1} \approx U(U^TJ_g^T\Sigma^-_{t+1} J_gU + S_R)^{-1}U^T
\end{equation}

where $S_R$ contains the top-most singular values of $R$. For simplicity, the state prediction covariance $Q$ was approximated as $Q=\gamma I_{n\times n} $, where $\gamma \in \mathbb{R}$.

We assume that ground-truth state measurements of $x_t$ are available during data collection. The observation model is then trained on $(x_t:y_t)$ pairs. During testing, the direct state measurements are either unavailable or unreliable.

==> future_work.tex <==
\section{Future Work}

In training our models on state-observation pairs, we have assumed that ground-truth state measurements are reliably obtained from joint encoders through low-velocity operation. In future work, training data will be collected using a high-fidelity motion-capture system to collect ground-truth joint displacement values. New data sets will also be comprised of scenes containing partial or total occlusion of the manipulator, to further demonstrate the tracking performance of the framework.


% We also anticipate extending the state-space to include up to 7 degrees-of-freedom, using all available joints in the robotic arm. New data sets will also be comprised of scenes containing partial or total occlusion of the manipulator. 
% Lastly, future results will include comparisons to generative models trained using adversarial methods, given recent successes of such approaches in the literature.


==> trans_model.tex <==
\section{Transition Model}


\textbf{Kinematic models}

\begin{itemize}
    \item 1st-order
    \begin{itemize}
    \item $ \dot{x}_{t} = x_{t} - x_{t-1} $\\
        $ x_{t+1} = x_{t} + \dot{x} \Delta t$
         $ x_{t+1} = x_{t} + \left(x_{t} - x_{t-1}\right) \Delta t$
    \item Assumes constant time-step: $ \Delta t = T $
    \end{itemize}
\end{itemize}


\textbf{Dynamics models}

Maps joint torques, velocity, and position at time $t$ to velocity and position at time $t+1$.
% True EKF would use a nonlinear model. 

\begin{itemize}
    \item Neural Network

    \item Analytic robot dynamics model
    % Show equations

\end{itemize}







